Magnetic and Transport Properties of (La,Sr)MnO$_3$

Magnetic and transport properties of the perovskite-type $3d$ transition-metal oxide (La,Sr)MnO$_3$ are theoretically studied using the double-exchange model in infinite dimension. Magnetoresistance properties as well as the magnetic transition temperatures are in good agreement with the experimental data.

==> iklfig.tex <==
%auto-ignore
\begin{figcaption}

\item Curie Temperature as a function of doping.
\label{FigTc}

\item Resistivity as a function of 
 spontaneous magnetization and 
field-induced magnetization.
%The experimental data  are taken from ref.~\cite{Tokura94}.
\label{FigMR}


\end{figcaption}
%

